$\text{Memory}^3$: Language Modeling with Explicit Memory

The training and inference of large language models (LLMs) are together a costly process that transports knowledge from raw data to meaningful computation. Inspired by the memory hierarchy of the human brain, we reduce this cost by equipping LLMs with explicit memory, a memory format cheaper than model parameters and text retrieval-augmented generation (RAG). Conceptually, with most of its knowledge externalized to explicit memories, the LLM can enjoy a smaller parameter size, training cost, and inference cost, all proportional to the amount of remaining "abstract knowledge". As a preliminary proof of concept, we train from scratch a 2.4B LLM, which achieves better performance than much larger LLMs as well as RAG models, and maintains higher decoding speed than RAG. The model is named $\text{Memory}^3$, since explicit memory is the third form of memory in LLMs after implicit memory (model parameters) and working memory (context key-values). We introduce a memory circuitry theory to support the externalization of knowledge, and present novel techniques including a memory sparsification mechanism that makes storage tractable and a two-stage pretraining scheme that facilitates memory formation.

==> Chapters/0._Frontpage.tex <==
\begin{titlepage}

\centering

\begin{tikzpicture}

\node[opacity=0.2,inner sep=0pt,remember picture,overlay] at (4.5,-0.5){\includegraphics[width= 0.8 \textwidth]{Figures/Decoration/us-giraldillo-grey.png}};

\node[inner sep=0pt] (logo) at (0,0)
    {\includegraphics[width=.25\textwidth]{Figures/Decoration/logo.png}};
    
\node[text width = 0.5\textwidth, right = of logo](title){\sffamily\huge\reporttitle};

\node[text width = 0.5\textwidth, yshift = 0.75cm, below = of title](subtitle){\sffamily\Large \reportsubtitle};
1
\gettikzxy{(subtitle.south)}{\sffamily\subtitlex}{\subtitley}
\gettikzxy{(title.north)}{\titlex}{\titley}
\draw[line width=1mm, Tue-red]($(logo.east)!0.5!(title.west)$) +(0,\subtitley) -- +(0,\titley);

\end{tikzpicture}
\vspace{3cm}

xxx,xxx,xxxx,xxxx \\
Department of LLM  \\
Institute for Advanced Algorithms Research, Shanghai\\
xxx@iaar.ac.cn


\tikz[remember picture,overlay]\node[anchor=south,inner sep=0pt] at (current page.south) {\includegraphics[width=\paperwidth]{Figures/Decoration/us-bg.jpg}};

\mbox{}
\vfill
\sffamily \Large \textcolor{white}{\placeanddate} \\



\end{titlepage}










==> Chapters/Z._Template.tex <==
\section{Introduction} \pagenumbering{roman}
xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 











% \subsubsection{This is a subsubsection}
% This section contains some templates that can be used to create a uniform style within the document. It also shows of the overall formatting of the template, created using the predefined styles from the \texttt{settings.tex} file.

% \subsection{General formatting}
% Firstly, the document uses the font mlmodern, using no indent for new paragraphs and commonly uses the color \textcolor{Tue-red}{Tue-red} (the color of the TU/e logo) in its formatting. It uses the \texttt{fancyhdr} package for its headers and footers, using the TU/e logo and report title as the header and the page number as the footer. The template uses custom section, subsection and subsubsection formatting making use of the \texttt{titlesec} package.\\
% The \texttt{hyperref} package is responsible for highlighting and formatting references like figures and tables. For example \cref{table: style 1} or \cref{fig: three images}. It also works for citations \cite{texbook}. Note how figure numbers are numbered according to the format \texttt{<chapter number>.<figure number>}.\\

% Bullet lists are also changed globally, for a maximum of 3 levels:

% \begin{itemize}
%     \item Item 1
%     \item Item 2
%     \begin{itemize}
%         \item subitem 1
%         \begin{itemize}
%             \item subsubitem 1
%             \item subsubitem 2
%         \end{itemize}
%     \end{itemize}
%     \item Item 3
% \end{itemize}

% Similarly numbered lists are also changed document wide:

% \begin{enumerate}
%     \item Item 1
%     \item Item 2
%     \begin{enumerate}
%         \item subitem 1
%         \begin{enumerate}
%             \item subsubitem 1
%             \item subsubitem 2
%         \end{enumerate}
%     \end{enumerate}
%     \item Item 3
% \end{enumerate}

% \newpage

% \subsection{Tables and figures}
% The following table, \cref{table: style 1}, shows a possible format for tables in this document. Alternatively, one can also use the black and white version of this, shown in \cref{table: style 2}. Note that caption labels are in the format \textbf{\textcolor{Tue-red}{Table x.y:} }
% \begin{table}[ht]
% \rowcolors{2}{Tue-red!10}{white}
% \centering
% \caption{A table without vertical lines.}
% \begin{tabular}[t]{ccccc}
% \toprule
% \color{Tue-red}\textbf{Column 1}&\color{Tue-red}\textbf{Column 2}&\color{Tue-red}\textbf{Column 3}&\color{Tue-red}\textbf{Column 4}&\color{Tue-red}\textbf{Column 5}\\
% \midrule
% Entry 1&1&2&3&4\\
% Entry 2&1&2&3&4\\
% Entry 3&1&2&3&4\\
% Entry 4&1&2&3&4\\
% \bottomrule
% \end{tabular}
% \label{table: style 1}
% \end{table}

% \begin{table}[ht]
% \rowcolors{2}{gray!10}{white}
% \centering
% \caption{A table without vertical lines.}
% \begin{tabular}[t]{ccccc}
% \toprule
% \textbf{Column 1}&\textbf{Column 2}&\textbf{Column 3}&\textbf{Column 4}&\textbf{Column 5}\\
% \midrule
% Entry 1&1&2&3&4\\
% Entry 2&1&2&3&4\\
% Entry 3&1&2&3&4\\
% Entry 4&1&2&3&4\\
% \bottomrule
% \end{tabular}
% \label{table: style 2}
% \end{table}

% For normal, single image figures, the standard \texttt{\textbackslash begin\{figure\}} environment can be used. For multi-image figures, one could use either the \texttt{\textbackslash begin\{subfigure\}} environment to get a main caption with 3 subcaptions like \cref{fig: three images} or the \texttt{\textbackslash begin\{minipage\}} environment to get 3 independent captions like \cref{fig: style 2 image a} - \ref{fig: style 2 image c}

% \begin{figure}[H]
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{example-image-a}
%          \caption{image a}
%          \label{fig: style 1 image a}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{example-image-b}
%          \caption{image b}
%          \label{fig: style 1 image b}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{example-image-c}
%          \caption{image c}
%          \label{fig: style 1 image c}
%      \end{subfigure}
%         \caption{Three images}
%         \label{fig: three images}
% \end{figure}

% \begin{figure}[H]
% \centering
% \begin{minipage}{0.3\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{example-image-a}
%   \captionof{figure}{image a}
%   \label{fig: style 2 image a}
% \end{minipage}
% \hfill
% \begin{minipage}{0.3\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{example-image-b}
%   \captionof{figure}{image b}
%   \label{fig: style 2 image b}
% \end{minipage}
% \hfill
% \begin{minipage}{0.3\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{example-image-c}
%   \captionof{figure}{image c}
%   \label{fig: style 2 image c}
% \end{minipage}
% \end{figure}
